Reward Uncertainty for Exploration in Preference-based Reinforcement Learning

Conveying complex objectives to reinforcement learning (RL) agents often requires meticulous reward engineering. Preference-based RL methods are able to learn a more flexible reward model based on human preferences by actively incorporating human feedback, i.e. teacher's preferences between two clips of behaviors. However, poor feedback-efficiency still remains a problem in current preference-based RL algorithms, as tailored human feedback is very expensive. To handle this issue, previous methods have mainly focused on improving query selection and policy initialization. At the same time, recent exploration methods have proven to be a recipe for improving sample-efficiency in RL. We present an exploration method specifically for preference-based RL algorithms. Our main idea is to design an intrinsic reward by measuring the novelty based on learned reward. Specifically, we utilize disagreement across ensemble of learned reward models. Our intuition is that disagreement in learned reward model reflects uncertainty in tailored human feedback and could be useful for exploration. Our experiments show that exploration bonus from uncertainty in learned reward improves both feedback- and sample-efficiency of preference-based RL algorithms on complex robot manipulation tasks from MetaWorld benchmarks, compared with other existing exploration methods that measure the novelty of state visitation.

==> sections/abstract.tex <==
Conveying complex objectives to reinforcement learning (RL) agents often requires meticulous reward function design and engineering. Preference-based RL methods are able to learn a more flexible reward model based on human preferences by actively incorporating human feedback, i.e. teacher preferences between two clips of behaviors.
However, feedback-efficiency still remains to be a limitation in current preference-based RL algorithms, as tailored human feedback is very expensive.
In order to address this challenge, previous improvements have mainly focused on methods to select informative queries and  improve policy initialization.
At the same time, recent exploration methods have proven to be a recipe for improving sample-efficiency in deep reinforcement learning (RL).
We present an exploration method specifically for preference-based RL algorithms. We utilizes disagreement in learned reward model ensemble predictions as intrinsic reward. Since we observe uncertainty-based query selection methods perform better than uniform random sampling strategies in complex tasks, our intuition is that disagreement in learned reward model reflects uncertainty in tailored human feedback and could be useful for exploration.
Our experiments show that reward uncertainty exploration improves both feedback- and sample-efficiency of preference-based RL algorithms on complex robot manipulation tasks from Meta-World benchmarks, compared with other existing exploration methods in traditional deep RL setting.

==> sections/discussion.tex <==
In this paper, we present RUNE, a simple and efficient exploration method specifically for preference-based RL algorithms. To improve sample- and feedback-efficiency of preference-based RL, different from previous works, we investigate the benefits of exploration methods in preference-based RL algorithms. We show the significant potential of incorporating intrinsic rewards to drive exploration because it improves sample-efficiency of preference-based RL.
For our proposed exploration scheme RUNE, we show that is suitable for preference-based RL because it showcases consistently superior performance in both sample- and feedback-efficiency compared to other existing exploration methods. Here we emphasize that RUNE, for the first time, takes advantage of information in reward functions learned from human feedbacks, to measure the novelty of states and actions for exploration. This is fundamentally different from other existing estimates of uncertainty for exploration as it in particular encourages exploration aligned to teacher preferences.
In conclusion, we hope that our work could demonstrate the potential of exploration to improve sample- and feedback-efficiency of preference-based RL, and to encourage developing novel exploration methods guided by human feedback.
